DYNAMO-HST Survey: Clumps in Nearby Massive Turbulent Disks and the Effects of Clump Clustering on Kiloparsec Scale Measurements of Clumps

We present $\sim$100 pc resolution Hubble Space Telescope H$\alpha$ images of 10 galaxies from the DYnamics of Newly-Assembled Massive Objects (DYNAMO) survey of low-$z$ turbulent disk galaxies, and use these to undertake the first detailed systematic study of the effects of resolution and clump clustering on observations of clumps in turbulent disks. In the DYNAMO-{\em HST} sample we measure clump diameters spanning the range $d_{clump} \sim 100-800$~pc, and individual clump star formation rates as high as $\sim5$~M$_{\odot}$~yr$^{-1}$. DYNAMO clumps have very high SFR surface densities, $\Sigma_{SFR}\sim 15$~M$_{\odot}$~yr$^{-1}$~kpc$^{-2}$, $\sim100\times$ higher than in H{\sc ii} regions of nearby spirals. Indeed, SFR surface density provides a simple dividing line between massive star forming clumps and local star forming regions, where massive star forming clumps have $\Sigma_{SFR}> 0.5$~M$_{\odot}$~yr$^{-1}$~kpc$^{-2}$. When degraded to match the observations of galaxies in $z\sim 1-3$ surveys, DYNAMO galaxies are similar in morphology and measured clump properties to clumpy galaxies observed in the high-$z$ Universe. Emission peaks in the simulated high-redshift maps typically correspond to multiple clumps in full resolution images. This clustering of clumps systematically increases the apparent size and SFR of clumps in 1~kpc resolution maps, and decreases the measured SFR surface density of clumps by as much as a factor of 20$\times$. From these results we can infer that clump clustering is likely to strongly effect the measured properties of clumps in high-$z$ galaxies, which commonly have kiloparsec scale resolution.

==> binhex.tex <==
%%
%% This is file `binhex.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% binhex.dtx  (with options: `style')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from binhex.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file binhex.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\next{\toks0=%
   {\catcode`\noexpand\@=\the\catcode`\@\toks0{\the\toks0}}%
}
\next
\catcode`\@11
\def\next#1#2#3{\expandafter \def \csname bb@#1\endcsname##1%
  {#2\csname bb@#3##1\endcsname}}
\next{00}00 \next{01}01 \next{02}10 \next{03}11
\next{04}20 \next{05}21 \next{06}30 \next{07}31
\next{08}40 \next{09}41 \next{10}50 \next{11}51
\next{12}60 \next{13}61 \next{14}70 \next{15}71
\next{16}80 \next{17}81 \next{18}90 \next{19}91
\expandafter \def \csname bb@0+\endcsname {+0}
\expandafter \def \csname bb@1+\endcsname {+1}
\def\bb@endbinary#1+{\fi\fi}
\expandafter \def \csname bb@0-\endcsname {0+-\bb@dobinary}
\expandafter\def\csname bb@0m\endcsname#1+{#1+0}
\expandafter\def\csname bb@1m\endcsname#1+{#1+1}
\def\bb@dobinary#1#2{\if#10\if m\string#2\else\bb@endbinary\fi\fi
 \expandafter\bb@dobinary\number\csname bb@0#1\endcsname#2}
\def\nbinary#1#2{\expandafter\bb@dobinary\number\number#2%
 \romannumeral\number\number#1 000+}
\def\binary{\nbinary1}
\def \next #1#2{\expandafter \def
 \csname bb@h\number +#1\endcsname ##1+{\bb@dohex ##1+#2}%
}
\next   {0}0 \next   {1}1 \next  {10}2 \next  {11}3
\next {100}4 \next {101}5 \next {110}6 \next {111}7
\next{1000}8 \next{1001}9 \next{1010}A \next{1011}B
\next{1100}C \next{1101}D \next{1110}E \next{1111}F
\def\bb@dohex #1{\csname bb@x#1\endcsname}
\def\bb@x\endcsname#1{ \bb@xm{m\endcsname}}
\def\bb@xm #1\endcsname #2#3+{#2#3%
 \csname bb@h\number+\endcsname
 #1\endcsname m#3+}
\def\bb@nbinbased #1#2#3{\expandafter \bb@dobinary \number#1%
 \expandafter \bb@dohex
 \romannumeral \number\number #2 000\expandafter\endcsname
 \romannumeral \number\number #3 000+}
\def\nbinbased #1#2#3{\expandafter\bb@nbinbased
 \expandafter {\number#3}{#2}{#1}}
\def\nhex{\nbinbased4}
\def\noct{\nbinbased3}
\def\ntetra{\nbinbased2}
\def\hex{\nhex1}
\def\oct{\noct1}
\def\tetra{\ntetra1}
\the\toks0
\endinput
%%
%% End of file `binhex.tex'.

